Type-Aware Decomposed Framework for Few-Shot Named Entity Recognition

Despite the recent success achieved by several two-stage prototypical networks in few-shot named entity recognition (NER) task, the overdetected false spans at the span detection stage and the inaccurate and unstable prototypes at the type classification stage remain to be challenging problems. In this paper, we propose a novel Type-Aware Decomposed framework, namely TadNER, to solve these problems. We first present a type-aware span filtering strategy to filter out false spans by removing those semantically far away from type names. We then present a type-aware contrastive learning strategy to construct more accurate and stable prototypes by jointly exploiting support samples and type names as references. Extensive experiments on various benchmarks prove that our proposed TadNER framework yields a new state-of-the-art performance. Our code and data will be available at https://github.com/NLPWM-WHU/TadNER.

==> sections/ethics_statement.tex <==
\section*{Ethics Statement}
Our work is entirely at the methodological level and therefore there will not be any negative social impacts. 
In addition, since the performance of the model is not yet at a practical level, it cannot be applied in certain high-risk scenarios (such as the I2B2 dataset used in our paper) yet, leaving room for further improvements in the future.


